Deconfinement critical point of lattice QCD with $N_{\rm f}=2$ Wilson fermions

The ${\rm SU}(3)$ pure gauge theory exhibits a first-order thermal deconfinement transition due to spontaneous breaking of its global $Z_3$ center symmetry. When heavy dynamical quarks are added, this symmetry is broken explicitly and the transition weakens with decreasing quark mass until it disappears at a critical point. We compute the critical hopping parameter and the associated pion mass for lattice QCD with $N_f=2$ degenerate standard Wilson fermions on $N_\tau\in\{6,8,10\}$ lattices, corresponding to lattice spacings $a=0.12\, {\rm fm}$, $a=0.09\, {\rm fm}$, $a=0.07\, {\rm fm}$, respectively. Significant cut-off effects are observed, with the first-order region growing as the lattice gets finer. While current lattices are still too coarse for a continuum extrapolation, we estimate $m_\pi^c\approx 4 {\rm GeV}$ with a remaining systematic error of $\sim 20\%$. Our results allow to assess the accuracy of the LO and NLO hopping expanded fermion determinant used in the literature for various purposes. We also provide a detailed investigation of the statistics required for this type of calculation, which is useful for similar investigations of the chiral transition.

==> kappa_table.tex <==
\begin{table*}[t]
    \setlength{\tabcolsep}{1pt}
    \renewcommand{\arraystretch}{1.0}
    \centering
\begin{tabular}{| c | c | c | c | c | c |}
\hline
\diagbox[height=0.6cm,width=0.9cm]{$N_s$}{$\kappa$} & 0.0750 & 0.0850 & 0.0900 & 0.1000 & 0.1100 \\ \hline 
$30$ & \cellcolor{gray!40} &  \cellcolor{gray!40} & \cellcolor{green!20} &  \cellcolor{green!20}& \cellcolor{green!20}\\ \hline
$36$ & \cellcolor{gray!40} &  \cellcolor{green!20} & \cellcolor{green!20} &  \cellcolor{green!20}& \cellcolor{green!20}\\ \hline
$42$ & \cellcolor{gray!40} &  \cellcolor{green!20} & \cellcolor{green!20} &  \cellcolor{green!20}& \cellcolor{green!20}\\ \hline
\end{tabular}
\caption{Example of $N_s$ - $\kappa$ table used for systematically excluding data points in the Binder fits.}
\label{tab:python_gui_nt6}
\end{table*}

